The role of magnetic fields in the formation of protostars, disks, and outflows

We present our current understanding of the formation and early evolution of protostars, protoplanetary disks, and the driving of outflows as dictated by the interplay of magnetic fields and partially ionized gas in molecular cloud cores. In recent years, the field has witnessed enormous development through sub-millimeter observations which in turn have constrained models of protostar formation. As a result of these observations % that the observations provided, the state-of-the-art theoretical understanding of the formation and evolution of young stellar objects is described. In particular, we emphasize the importance of the coupling, decoupling, and re-coupling between weakly ionized gas and the magnetic field on appropriate scales. This highlights the complex and intimate relationship between gravitational collapse and magnetic fields in young protostars.

==> sec_abstract.tex <==
We present our current understanding of the formation and early evolution of protostars, protoplanetary disks, and the driving of outflows and jets dictated by the interplay of  magnetic field and partially ionized gas in molecular cloud core.
In recent years, the field has witnessed massive development in the sub-millimeter observations and has constrained theoretical models of protostar formation. 
Under these observational constraints% that the observations provided,
the state-of-the-art theoretical understanding for the formation and evolution of young stellar objects is described.
In particular, we emphasize the importance of the coupling, decoupling, and recoupling between weakly ionized gas and magnetic field at appropriate scales. This highlights the complex and intimate relationship between gravitational collapse and the magnetic fields in young protostars.



==> sec_masahiro_old.tex <==
\subsubsection{Outflow/jet launching from newly born disk and protostar}
\label{Outflow_Theory}
Protostellar outflows and jets have been ubiquitously observed in star-forming regions. 
Thus, it is considered that they are proof of ongoing star formation and a new-born star is embedded in the root of each flow. 
These flows have various morphologies and typical velocities (see also \ref{SR_MHD_Outflows}). 
We observe wide-angle and slow-velocity flows called `molecular outflow' or `low-velocity outflow' in molecular line emissions.
On the other hand, well-collimated high-velocity flows called `collimated jet' or `optical jet' are observed by molecular and atomic line emissions from radio to optical wavelengths. The rest of this subsection, we call the former `the outflow' and the latter `the jet.'


The outflow and jet give significant impacts on the star formation because they directly transport
angular momentum and expel a large fraction of the infalling gas from the star-forming core. 
Observations have shown that the outflow momentum flux (the outflow momentum divided by the outflow dynamical timescale)
is much stronger  than the radiation force (or radiation pressure),
indicating that the protostellar luminosity is not sufficient to drive the flows \citep{1996A&A...311..858B,2004A&A...426..503W}.
As the driving mechanism of the flows, magnetically driven wind scenarios have been proposed \citep[e.g.,][]{1986ApJ...301..571P} and investigated in past theoretical and simulation studies, in which the outflow and jet are magnetocentrifugally driven \citep{1982MNRAS.199..883B}
or driven by magnetic pressure gradient force \citep{1985PASJ...37..515U}. 
%%\citet{1986ApJ...301..571P} showed the detailed picture of the outflow and jet to explain observational characteristics in their analytical study. 
However, the settings for driving the outflow and jet were highly idealized in past studies.
%%In other words, only conveniently conditions are used both for analytical and simulation studies.  
For example, considerably idealized (or an unrealistic) circumstellar disk and magnetic field configuration
such were prepared for the emergence of winds. 
For example, only poloidal fields (or dipole magnetic fields) were assumed within a thin disk as the initial state in past studies.   
The problem that such an idealized condition is actually realized in the star formation process. 
%\bc{I would add more details on the idealized condition (e.g. thin disk, poloidal fields}
%%at those days, researchers have concern about the artificially prepared   i.e., such idealized environment is realized in actual star formation, or outflow continues to be driven after its emergence. 
%%by the driving condition of jet is elaborately investigated both in analytical and simulation studies with highly idealized setting of which accretion disk penetrated by inclined magnetic field lines are prepared. 

For the first time,  \citet{1998ApJ...502L.163T,2000ApJ...528L..41T,2002ApJ...575..306T} could successfully reproduce
the outflow in the star formation simulation with a two dimensional ideal MHD code. 
He simulated the gravitational collapse process of star forming cores spatially resolving both prestellar core and protostar.
In his simulation, the outflow and jet naturally appear in gravitationally collapsing clouds. 
Then, driving the outflow and jet has been comprehensively investigated in many star-formation simulations \citep{2004MNRAS.348L...1M,2006ApJ...647L.151M,2006ApJ...641..949B,2008ApJ...676.1088M,2008A&A...477...25H,2010MNRAS.409L..39C,2011MNRAS.417.2036B,2012MNRAS.422..347S,2012MNRAS.423L..45P,2012A&A...543A.128J,2013ApJ...763....6T,2014MNRAS.437...77B,2017MNRAS.467.3324L,2018MNRAS.475.1859W,2018A&A...620A.182K,2021MNRAS.502.4911X}.
With these simulations, the driving mechanism of outflow and jet in the star formation process could be  established. 

%\bc{\sout{Star formation begins with the gravitational collapse of a molecular cloud core. 
%The first hydrostatic core forms in the gravitationally collapsing core when the central number density exceeds $\sim10^{10}$\,cm$^{-3}$.}} 
In a first core, the gravitational collapse slows and the collapse timescale is longer
than the rotation timescale.
%after the first hydrostatic core (hereafter the first core) formation.
Thus, magnetic field lines are twisted around the first core, and the low-velocity outflow emerges. 
The outflow emerged from the first core was recently confirmed in the ALMA observation
\citep{2015A&A...577L...2G,2020ApJ...899L..10F}.
%\bc{There is also the work by Gerin et al. 2016 on B1b}

%\bc{The processes described in the paragraph are already explained in the previous section $\rightarrow$ I deleted this paragraph.}

%%The angular momentum of the first core is effectively transported by the outflow \citep{2000ApJ...528L..41T}, while the magnetic field dissipates due to very low ionization degree inside the first core \citep{2008ApJ...676.1088M}. 
%%Therefore, the Lorentz and centrifugal forces weaken and the gravitational collapse is promoted  with the dissociation of hydrogen molecules and a protostar forms within the first  core. 
%%The magnetic field is coupled with the neutral gas again around the protostar due to the high temperature.
%%Thus, the magnetic field lines are strongly twisted and the magnetic field is significantly amplified.
%%Then, another component of the flow corresponding to the high-velocity jet appears near the protostar, as seen in Figure~\ref{fig:schematic}.

%%\begin{figure}
%%\begin{center}
%%%\includegraphics[width=62mm]{schematic.eps}
%%\caption{
%%%Schematic view of outflow and jet system constructed by core collapse simulations. %%\bc{Maybe add some scales in AU.}
%%}
%%\label{fig:schematic}
%%\end{center}
%%\end{figure}

%%Although the first core slightly shrinks after protostar formation, it evolves into a rotationally supported disk 
%\bc{As discussed, unclear to me. With top hat initial conditions, disk can form around the first core (Masson 2016). I mean it is was the case, the total mass disc plus first core sould be almost constant after disk formarion. I should check this. $\rightarrow$ I deleted the corresponding sentence because this point is wroted in previous section}.
The outflow driven by the first core before protostar formation continues
to be driven by the rotationally supported disk after protostar formation. 
Since the high-velocity jet is also driven near the inner edge of the disk, two flow components (i.e., outflow and jet) coexist.
%%(Fig.~\ref{fig:schematic}). 
The former corresponds to (wide-angle, low-velocity) molecular outflows, while the latter is (collimated high-velocity) optical jets. 
During the main accretion phase, gravitational instability occurs and the non-axisymmetric (or spiral structure) develops in the disk  \citep{2010ApJ...718L..58I}.  
Thus, the disk gas intermittently falls onto the protostar, inducing an episodic mass ejection or time-variable jet \citep{2019ApJ...876..149M}. 
The outflow physical parameters such as outflow mass, momentum, momentum flux, kinetic energy and kinetic luminosity are well agreement with observations, indicating that the molecular outflow is directly driven by the disk \citep[e.g.,][]{2013MNRAS.431.1719M}. 

The difference in velocity between the outflow and jet is due to the difference in driving radius. 
The outflow driven by the disk outer edge where the escape or Keplerian velocity is slow, while the jet is driven by the disk inner edge where the Keplerian velocity is high. 
No wind appears in the disk intermediate region where magnetic field and gas are decoupled.
The difference in morphology between them is related to the configuration and strength of magnetic field. 
A wire-like radially distributed fields guide the outflow  which is mainly driven by the magnetocentrierugal mechanism and creates a wide opening angle flow.

On the other hand,  weak fields that have experienced Ohmic dissipation and ambipolar diffusion
are passively twisted by the rotation of protostar and disk inner edge and generate a strong magnetic pressure gradient force to drive the jet.
Figure \ref{fig_protostar} illustrates this evolution.
The left panel shows the magnetic field configuration around the protostar
just after its formation in the ideal MHD simulation, and shows that an hourglass-shaped magnetic field has been realized.
This indicates that the strong magnetic field suppresses
the gas rotation and that the gas motion can not twist the magnetic field.
On the other hand, the weak magnetic field due to the magnetic diffusion
is easily twisted during the second collapse.
The middle panel shows the magnetic field configuration in the non-ideal MHD simulation,
and shows that the magnetic field is passively twisted by the rotation.
This passive twisting of the magnetic field drives the jets from the vicinity of the protostar, as shown in the right panel.
Therefore, magnetic diffusions also play an essential role in driving a protostellar jet.

Since the magnetic filed lines are strongly twisted inside the  jet, the hoop stress further improves the jet collimation \citep{2008ApJ...676.1088M}. 
The mass-loss rate of the jet obtained from the 3D simulation is $\sim 10^{-5}~\msunyear$ \citep{2019ApJ...876..149M}, and 
is in agreement with the observed value of protostar, $\sim 3 \times 10^{-6}~\msunyear$  \citep{2020A&ARv..28....1L}.

At last, we comment on the classical scenario for driving the outflow. 
It had been considered that the low-velocity outflow is entrained by the high-velocity (primary) jet (so-called the entrainment scenario). 
In this scenario, the jet appeared near the protostar provides linear momentum to the ambient gas through some mechanism \citep{2007prpl.conf..245A}. 
Then, the ambient gas entrained by the jet is observed as the low-velocity outflow. 
Recently, observations of the outflow rotation could resolve this long-standing debate on the outflow driving. 
It had been considered that we would unveil the outflow driving mechanism if the outflow rotation could be measured. 
In the entrainment scenario, the primary jet, which provides both linear and angular momentum to the outflow (or the entrained gas), has only a small amount of angular momentum, because the jet driving region is located near the protostar.
%% and the distance between the protostar and jet launching radius is not large.
Thus, it is expected that the outflowing gas receives a very small amount of angular momentum from the primary jet. 
On the other hand, in the direct disk driven scenario proposed from the core collapse simulations,
the outflow should have a large amount of angular momentum because the outflow driving region
is much far from the protostar where the rotation velocity and angular momentum are large. 

Before the ALMA era, researchers could not clearly confirm the outflow rotation because
the outflow gradually widens as it propagates into the infalling envelope and the rotation velocity decreases according to the angular momentum conservation law. 
Thus, we need to resolve the outflow driving region to detect the outflow rotation. 
In the ALMA era, \citet{2017NatAs...1E.146H} observed the outflow rotation for Orion Source I.
Then, based on the Bernoulli's theorem and the angular momentum conservation law,
they estimated the outflow launching radius much far from the protostar $\gtrsim 10$\,au \citep[see also][]{2016Natur.540..406B}. 
It should be noted that the configuration of magnetic field inside the outflow was also detected for Orion Soure I \citep{2020ApJ...896..157H}.
After the discovery, the outflow rotation was confirmed by ALMA for many objects \citep[e.g.][]{2016ApJ...824...72C,2018A&A...618A.120L,2018ApJ...856...14L,2021ApJ...916...23M}.
In addition, \citet{2017A&A...603L...3A} could resolve the outflow launching region which is located at the outer edge of the disk.
\citet{2019ApJ...871..221M} showed that the high-velocity jet axis is significantly
inclined from the low-velocity outflow axis, indicating that the launching radii of the high- and low-velocity components differ in an inclined disk. 
These recent observations support the direct disk wind expected from core collapse simulations. 
Although classical entrainment scenario is rejected by both recent theoretical and observation
studies, a part of gas can be entrained by the flow driven by various radii \citep{2021ApJ...907L..41L}. 

%\bc{At the end of section 3.1, I would add a dedicated section which recalls the main achievement of non-ideal MHD models. It can solve indeed the angular momentum and magnetic flux problems. It also reproduce the outflow and jet launching. But the question is now about disk evolution. Is has been shown that disks can form around the first (currently missing in the text) and second Larson cores, but we do not know how the two are connected and how they will evolve. In addition, the disk around the first and second core are very different (vertical versus toroidal fields). So long time evolution is required, as well as parameter space exploration. The above mentioned results all considered the aligned case which is very particular. This is what we discuss in the following section.}

